A constant factor approximation for Nash social welfare with subadditive valuations

We present a constant-factor approximation algorithm for the Nash social welfare maximization problem with subadditive valuations accessible via demand queries. More generally, we propose a template for NSW optimization by solving a configuration-type LP and using a rounding procedure for (utilitarian) social welfare as a blackbox, which could be applicable to other variants of the problem.

==> XOS_algorihm.tex <==
\section{Algorithm for NSW with XOS valuations}

In this section, we present a constant factor approximation algorithm for the Nash Social Welfare problem with XOS valuations in the demand oracle model. The problem is defined as follows

\paragraph{Nash Social Welfare (NSW).}
Given $m$ indivisible items and $n$ agents with valuation functions $v_i:2^{[m]} \rightarrow \RR_+$,
we want to allocate items to the agents, that is find a partition of the $m$ items $(S_1,S_2,\ldots,S_n)$ that maximizes the {\em geometric average} of the valuations,
$$ \NSW(S_1,S_2,\ldots,S_n) = \left( \prod_{i=1}^{n} v_i(S_i) \right)^{1/n}.$$

\paragraph{XOS (fractionally subadditive) functions.}
Let $\cG$ be a finite ground set. A valuation function $v: 2^\cG \to \RR$ is called XOS (or fractionally subadditive) if and only if there is a family of nonnegative additive functions $\cF$ such that $v(S) = \max_{f\in \cF} f(S)$ for every $S\subset\cG$. We call $\cF$ the XOS representation of $v$.

\paragraph{Demand oracle}
Let $\cG$ be a finite ground set and $v: 2^\cG \to \RR$. A demand oracle for $v$ is a black-box which takes a price vector $p \in \RR^{\cG}$ as input, and outputs a set $S\subset\cG$ that maximizes $v(S) - \sum_{i\in S}x_i$.

\begin{theorem}
\label{thm:XOS-alg}
There exists a polynomial-time constant-factor approximation algorithm for the Nash Social Welfare problem with XOS valuations, accessible by demand oracle queries
\end{theorem}

\begin{algorithm}[htbp]
\caption{\bf Nash Social Welfare algorithm}
\label{alg:NSW-template}
\begin{algorithmic}[1]
  \Procedure{NSW}{$\cA,\cG,v_1,\ldots,v_n$}:
    \State Find a matching $\tau:\cA \rightarrow \cG$ maximizing $\prod_{i \in \cA} v_i(\tau(i))$
    \State $\cH := \tau(\cA)$, $\cG' := \cG \setminus \cH$, $\cA' := \{i \in \cA: v_i(\cG') > 0\}$
    \State $\bx := $ {\bf ConfigurationLP}$(\cA',\cG',v_1,\ldots,v_n)$
    \State $\bx' := $ {\bf SetSplitting}$(\bx)$
    \State $(R_1,\ldots,R_n) := $ {\bf RandomizedRounding}$(\bx')$
    \State Find a matching $\sigma:\cA \rightarrow \cH$ maximizing $\prod_{i \in \cA} v_i(R_i + \sigma(i))$
    \State Return $(R_1 + \sigma(1), R_2 + \sigma(2), \ldots, R_n + \sigma(n))$
  \EndProcedure
\end{algorithmic}
\end{algorithm}

At a high level, we use a framework similar to the recent constant factor approximation algorithms for Rado \cite{GargHV21} and submodular \cite{LiV22} valuations.

\paragraph{Algorithm overview and comparison with the submodular case.} As the first step, we identify and reserve $n$ `high value' items by finding a matching $\tau:\cA \rightarrow \cG$ maximizing $\prod_{i \in \cA} v_i(\tau(i))$. 
Then we run a certain procedure to allocate the remaining items (and this procedure is the main new contribution of this work). At the end, we rematch the items in $\tau(\cA)$ based on how we allocated the remaining items. These first and last steps are essentially the same as in \cite{GargHV21,LiV22}, since they actually work even for  subadditive valuations. 

The challenges for XOS and subadditive valuations arise in the allocation of the remaining items. In the case of submodular valuations, the approach in \cite{LiV22} was to compute a fractional allocation based on the multilinear relaxation of the submodular optimization problem, and then round the solution probabilistically. However, for XOS valuations, the multilinear relaxation does not have the same concavity properties and we don't know how to solve the relaxation efficiently (even with demand oracles). Instead, we use a relaxation inspired by the Configuration LP for welfare maximization with demand oracles (see \cite{Feige09,FV10}, and also \cite{GargHV21}). Then we develop a novel rounding strategy for the NSW objective.


\subsection{The Eisenberg-Gale (log-concave) Relaxation}

We consider the following relaxation of the objective function $\prod_{i=1}^{n} v_i(S_i)$ of the Nash Social Welfare problem analogous to the relaxation in \cite{GargHV21, LiV22}: an optimization program which aims to assign the items in $\cH$ integrally and the remaining items fractionally under a certain relaxed objective.

\begin{align*}
\tag{Mixed-Concave}
\label{eqns:MM}
\max \quad & \prod_{i \in \cA} v_i^+(\bx_i) \\
s.t. \quad & \sum_{i\in\cA} x_{ij} \le 1 && \forall j\in \cG \\
& x_{ij} \ge 0 &&  \\
& x_{ij} \in \{0,1\} && \forall i \in \cA, j \in \cH
\end{align*}

where $ \forall i \in \cA'$,  $v_i^+(\bx_i)$ is the concave extension of the original discrete valuation $v_i$, defined as
\begin{align*}
\tag{Concave Extension}
\label{eqns:concave}
 & \max \sum_{S\subset\cG} v_i(S) x_{i,S} : \\
 &  \sum_{S \subset \cG:j\in S} x_{i,S} \le x_{ij} && \forall j\in \cG \\
 & \ \ \sum_{S\subset\cG} x_{i,S} = 1 \\
 & \ \  x_{i, S} \ge 0 &&  \forall S\subset\cG \\
\end{align*} 

Our relaxation is a natural modification of the Configuration LP for the Nash welfare objective: It uses a concave extension $v^+_i$ of the valuation function $v_i$ (which is known to be computable using demand queries \cite{Feige09,FV10}), and a summation of the logarithms of $v^+_i$ to reflect the NSW objective. In fact the relaxation for Rado valuations in \cite{GargHV21} happens to be a special case of this relaxation, although the relaxation in \cite{GargHV21} can be solved even using value queries, using either matroid properties or the gross substitutes property of Rado valuations. 

Let $\cG'$ be the set of unmatched items, $\cG' = \cG \setminus \cH$, and 
$\cA'$ be the subset of agents excluding those who don't derive any value from $\cG'$. We adopt a greedy method similar to \cite{GargHV21, LiV22} to solve the \ref{eqns:MM} relaxation approximately: first we try to allocate the items in $\cG' = \cG\setminus\cH$ based on the optimal fractional solution of the following concave program:

\begin{align*}
\tag{Log-Concave Relaxation}
\label{eqns:log-concave}
\max \quad & \sum_{i\in \cA'} \log v_i^+(\bx_i) \\
& \quad \sum_{i \in \cA'} x_{ij} \le 1 && \forall j \in \cG' \\
& \quad x_{ij} \ge 0 &&  \forall i \in \cA', j \in \cG' \\
\end{align*}

We can solve this relaxation based on the following lemma, which we prove in Appendix~\ref{app:solving-log-concave}.

\begin{lemma}
\label{lem:solving-log-concave} 
Given demand oracles for $v_1, \cdots, v_n$, an optimal solution $\bx^*$ for (Log-Concave Relaxation) can be found within any precision in polynomial time. Moreover, the support of $\bx^*$ has size polynomial in $n$.
\end{lemma}


Finally, we compute an optimal matching between $\cA$ and $\cH$ with respect to the allocation of items in $\cG'$.



\begin{comment}

Our relaxation is a natural modification of the Configuration LP for the Nash welfare objective: It uses a concave extension $v^+_i$ of the valuation function $v_i$ (which is known to be computable using demand queries \cite{Feige09,FV10}), and a summation of the logarithms of $v^+_i$ to reflect the NSW objective. In fact the relaxation for Rado valuations in \cite{GargHV21} happens to be a special case of this relaxation, although the relaxation in \cite{GargHV21} can be solved even using value queries, using either matroid properties or the gross substitutes property of Rado valuations. 

We describe the relaxation as follows. $\cG'$ here is the set of unmatched items, $\cG' = \cG \setminus \cH$, and 
$\cA'$ here is the subset of agents excluding those who don't derive any value from $\cG'$.

\begin{align*}
\tag{Log-Concave Relaxation}
\label{eqns:log-concave}
\max \quad & \sum_{i\in \cA'} \log v_i^+(\bx_i) \\
& \quad \sum_{i \in \cA'} x_{ij} \le 1 && \forall j \in \cG' \\
& \quad x_{ij} \ge 0 &&  \forall i \in \cA', j \in \cG' \\
\end{align*}
where $ \forall i \in \cA'$,
\begin{align*}
\tag{Concave Extension}
\label{eqns:concave}
 v_i^+(\bx_i) = & \max \sum_{S\subset\cG'} v_i(S) x_{i,S} : \\
 &  \sum_{S \subset \cG':j\in S} x_{i,S} \le x_{ij} && \forall j\in \cG' \\
 & \ \ \sum_{S\subset\cG'} x_{i,S} = 1 \\
 & \ \  x_{i, S} \ge 0 &&  \forall S\subset\cG' \\
\end{align*}

\begin{lemma}
\label{lem:solving-log-concave} 
Given demand oracles for $v_1, \cdots, v_n$, an optimal solution $\bx^*$ can be found within any precision in polynomial time. Moreover, the support of $\bx^*$ has size polynomial in $n$.
\end{lemma}

We prove this lemma in Appendix~\ref{app:solving-log-concave}.
\end{comment}


\subsection{Randomized Rounding}

Assuming that we can solve (Log-Concave Relaxation), our goal is to round the fractional solution. The most straightforward way is to sample a set $S_i$ for each agent according to the solution $x_{i,S}$ independently and then resolve conflicts between agents. Intuitively speaking, there is only a constant number of agents competing for any item in expectation, and therefore we should be able to recover a constant fraction of $v_i(S_i)$. 
%And if we restrict the valuations to any pair $(i, S)$ in the support of $\bx$, the value of any subset $S'$ is at least $f_{i,S}(S')$. Therefore we could assume the restricted valuations to be additive and then independently randomized rounding should resolve the conflict with good probability like \cite{LiV22}.

However, one issue here is that $x_{i, S}$ may induce a distribution of value $v_i(S_i)$ of large variation for each agent. In that case, allocating random sets according to $x_{i,S}$ might always give high value to some agents and low value to others, which hurts the NSW objective.
%For example, if a valuation function is additive, the Configuration LP can only control the marginal probabilities of items. It cannot distinguish between the product distribution and the case where all items appear together with a small probability. 
So our strategy is to first modify the distribution in such a way that the values of $v_i(S)$ in the support of $x_{i,S}$ are roughly equal. More specifically, we will discard those sets whose values are way below the average and split the remaining sets into pieces that have value roughly around the average.

Another issue is that the distribution of items arising from a contention resolution scheme is actually not independent between the items (due to correlated competition with other agents). We resolve this by considering a two-step procedure, where in the first step we consider a fractional allocation, divided uniformly among the competing agents for each item, and then we allocate items independently according to this fractional solution. Although this is just another equivalent way of viewing the same algorithm, we can invoke concentration bounds this way and prove that the Nash social welfare is good in expectation. 

We proceed to describe our algorithm in more detail.

\paragraph{SetSplitting($\bx$).}
Given an optimal solution $\bx$ to (Log-Concave Relaxation):
\begin{enumerate}
     \item Let $\cF_i = \{S\subset\cG': v_i(S)\ge \frac14 v_i^+(\bx_i)\}$ and for each $S \in \cF_i$, let $f_{i,S}$ be the additive function in the XOS representation of $v_i$ that defines the value of $v_i(S)$. Let $l_{i,S}$ be an item in $S$ with the largest value with respect to $f_{i,S}$. 

    \item Set $x'_{i, S} = 0$ and $k_{i,S} = 0$  for $S \notin \cF_i$; i.e., discard sets whose value is too low.
    
    \item For every $S \in \cF_i$, let $k_{i, S} = \lfloor 4 v_{i}(S)/v_i^+(\bx_i)\rfloor$, split $S - l_{i, S}$ into sets $S_1, \cdots, S_{k_{i, S}}$ such that $f_{i,S}(S_j + l_{i, S})\ge \frac14 v_i^+(\bx_i)$. (Note that this is possible since the average value of one of $k_{i,S}$ subsets in a partition of $S$ is $v_i(S) / k_{i,S} \geq \frac14 v^+_i(\bx)$, and the inclusion of $l_{i,S}$ compensates for rounding issues.)

    \item Set $x'_{i,T} = \frac34 \sum_{S \in \cF_i, j: T=S_j} x_{i,S}$.

    \item Return $\bx'$.
    
\end{enumerate}

%From the description, it is obvious that $v_i(S_j + l_{i, S})\ge \frac14 v_i^+(\bx_i)$ for any $S_j$ in the support of $\bx'_i$. %Also, the value of $\bx'$ can only increase compared to $\bx$, by subadditivity: $\sum_{j=1}^{k_{i,S}} v_i(S_j+l_{i,S}) \geq v_i(S_j+l_{i,S})$. 
%We also prove that the constraints are satisfied by $\bx'$ up to constant factors,  which is useful in the following.

The obtained fractional solution satisfies some useful properties, stated in the following lemma.

\begin{lemma}
\label{lem:x'-bounds}
    The fractional solution $\bx'$ returned by {\bf{SetSplitting}}($\bx$) satisfies that \\
    for any $S_j$ in the support of $\bx'_i$,
    $$v_i(S_j + l_{i, S})\ge \frac14 v_i^+(\bx_i);$$
    for any $i\in \cA'$,
    $$ 1 \le \sum_{S\subset \cG'} x'_{i, S} \le 3;$$ 
    and for any $j\in \cG'$,
    $$\sum_{i\in \cA', j\in S}x_{i, S}' \le \frac{3}{4}.$$
\end{lemma}
    
\begin{proof} 
    The first point is obvious from the construction.

    For the second point, recall that $\cF_i = \{S\subset\cG': v_i(S)\ge \frac12 v_i^+(\bx_i)\}$. First we prove the upper bound:
    $$\sum_{S\subset \cG'}x'_{i, S} = \frac34 \sum_{S \in \cF_i} k_{i,S} x_{i,S} = \frac34 \sum_{S \in \cF_i} \left\lfloor\frac{4 v_{i}(S)}{v_i^+(\bx_i)} \right\rfloor \cdot x_{i, S} \le 3 \sum_{S\subset \cG'}\frac{v_{i}(S) x_{i, S}}{v_i^+(\bx_i)} = 3.$$ 
    For the lower bound, we have 
    $$\sum_{S\in \cF_i} v_i(S)x_{i, S} = v_i^+(\bx_i) - \sum_{S\notin \cF_i} v_i(S)x_{i, S}\ge v_i^+(\bx_i) - \frac{1}{4} v_i^+(\bx_i) = \frac34 v_i^+(\bx_i),$$ 
    $$\sum_{S\subset \cG'}x'_{i, S} = \frac34 \sum_{S \in \cF_i} k_{i,S} x_{i,S} = \frac34 \sum_{S \in \cF_i} \left\lfloor\frac{4 v_{i}(S)}{v_i^+(\bx_i)} \right\rfloor \cdot x_{i,S} \ge \frac34 \sum_{S\in \cF_i}\frac{2 v_{i}(S)x_{i, S}}{v_i^+(\bx_i)} \geq 1 $$ 
    considering that $4 v_i(S) / v_i^+(\bx_i) \geq 1$ for $S \in \cF_i$, so the floor operation can decrease the ratio by at most a factor of $2$. Also, we have $\sum_{S \in \cF_i} v_i(S) x_{i,S} \geq \frac34 v^+_i(\bx_i)$ from above.

    Finally, observe that the coefficients $x'_{i,S}$ for sets containing any fixed item $j$ are at most $3/4$ times the corresponding coefficients $x_{i,S}$ containing the same item. Since the coefficients $x_{i,S}$ for $S$ containing $j$ add up to at most $1$, the coefficients $x'_{i,S}$ for $S$ containing $j$ add up to at most $3/4$.
\end{proof}



\paragraph{RandomizedRounding($\bx$)}

We use the following multi-step rounding scheme.

\begin{enumerate}
    \item For every $i\in \cA'$, find $c_i$ such that $c_i\sum_{S\subset \cG'} x'_{i, S} = 1$.

    \item For each agent $i$ independently, pick a tentative set $S_i$ with probability $c_i x'_{i, S_i}$. 

    \item Let $T_j$ be the set of agents whose tentative set contains item $j$. For each item $j$ independently, assign it to an agent in $T_j$ uniformly.
    
    \item Define $R_i = \{j \in \cG \setminus \cH: \mbox{agent $i$ gets item $j$}  \}$.

    \item Return $(R_1,\ldots,R_n)$.
\end{enumerate}


The following lemma shows that this procedure does not lose too much value; we note that the bound here is stronger than what we need to bound Nash social welfare, and similar to the quantity used in \cite{LiV22}. 
%Both the statement and the proof are similar to Lemma 5 in \cite{LiV22}.

Let $l_i$ and $f_i$ be the $l_{i,S}$ and $f_{i,S}$ from {\bf SetSplitting} with corresponding $S$ where $S_i$ is split from,
i.e, $f_i(A) = \sum_{j \in A} v_{ij}$. It should be clear from context which set we are talking about so we just omit it for simplicity. We can extend $f_i$ to vectors with real coordinates as follows: $$f_{i} : \bx_i \mapsto \sum_{j\in S} v_{ij} x_{ij} $$
(note that we only care about its behavior on $[0,1]^S$ for the corresponding $S$).


\begin{lemma}
\label{lem:rounding} For any feasible solution $\bx^*$ of (Log-Concave-relaxation), with constant probability, the solution $R$ obtained by {\bf RandomizedRounding} satisfies
$$\frac{1}{n} \sum_{i \in \cA'} \frac{v^+_i(\bx^*_i)}{v_i(R_i + l_{i})} \leq 90. $$
\end{lemma}

\begin{proof}  
Let $\bx$ be an optimal solution to (Log-Concave Relaxation) and $\bx^*$ any feasible solution (corresponding to the optimal solution overall). By Lemma~\ref{lem:local-opt}, we have
\begin{equation}
    \label{eq:local-opt-bound}
\sum_{i \in \cA'} \frac{v^+_i(\by^*_i)}{v^+_i(\by_i)} \leq 2 |\cA'| \leq 2n.
\end{equation} 

As described above, first we consider the rounding step 2 which samples a set $S_i$ for each agent $i$. Recall that $T_j = \{i: j \in S_i\}$ are the agents competing for item $j$. Also, the scaling factor $c_i$ used in Step 1 can be assumed to be in $[1/3,1]$, due to Lemma~\ref{lem:x'-bounds}. Hence $\sum_{i, S \ni j} c_i x'_{i,S} \leq 3/4$.

Define a fractional assignment $\by$ such that 
\begin{align*}
    y_{ij} = \left\{\begin{array}{cc}
        1 & \mbox{if } j = l_i  \\
        |T_j|^{-1} & \mbox{if } j\in S_i \\
        0 & \mbox{otherwise.} 
    \end{array}\right.
\end{align*}
Observe that 
$$\E[|T_j| \mid i\in T_j] = 1 + \sum_{i' \neq i, S \ni j} c_i x'_{i,S} \le 1 + 3/4 = 7/4$$ for any $j\in S_i$. We denote by $L_i$ the set $S_i\cup\{l_i\}$, by $f_i$ the additive function from the XOS representation of $v_i$ defining the value of $L_i$, and recall that the vector $\by_i$ always contains $1$ for the large item $l_i$.
By a comparison between the arithmetic and harmonic mean (with values $y_{ij}$ and weights $v_{ij} / \sum_{j \in S_i} v_{ij}$),  we have 
\begin{align*}
    f_{i}(\by_i) = \sum_{j\in L_i} v_{ij} y_{ij} &\ge \left(\sum_{j\in L_i}v_{iej} \right)\left(\sum_{j\in L_i}\frac{v_{ij}}{\sum_{j\in L_i}v_{ij}} y_{ij}^{-1}\right)^{-1} \\
    & = f_{i}(L_i)\left(\sum_{j\in L_i}\frac{v_{ij}}{\sum_{j\in L_i} v_{ij}} y_{ij}^{-1}\right)^{-1} \\
    & = v_{i}(L_i)\left(\sum_{j\in L_i}\frac{v_{ij}}{\sum_{j\in L_i} v_{ij}} y_{ij}^{-1}\right)^{-1}.
\end{align*} 
Conditioned on the choice of $S_i$ for agent $i$, the vector $\by$ is still random, depending through $|T_j|$ on the sets chosen by other agents. Hence, using the inequality above, we have
\begin{align*}
    \E\left[\frac{v^+_i(\bx)}{f_{i}(\by)} \Big| S_i \right] &\le \frac{v^+_i(\bx)}{v_{i}(L_i)} \ \E\left[\sum_{j\in L_i}\frac{v_{i, j}}{\sum_{j\in L_i}v_{i, j}} y_{ij}^{-1} \Big| S_i \right] \\ 
    &\le \frac{v^+_i(\bx)}{v_{i}(L_i)} \ \max_{j\in L_i}\E[|T_j| \mid i\in T_j] \\
    &\le 4 \times \frac{7}{4} = 7 
\end{align*}
using the computation above and the fact that after set splitting, $v_i(L_i) \geq \frac14 v_i^+(\bx_i)$.

In the following, we condition the sets sampled for all agents, and hence also the vector $\by$, without stating it explicitly in all expressions.
Observe that the set $R_i+l_i$ can be viewed as sampling elements independently with probabilities $y_{ij}$. 
By the Efron-Stein inequality, 
$$\Var\left[f_i(R_i + l_{i}) \right] \le \E\left[\sum_{j\in R_i}v_{ij}^2\right]\le \E\left[\sum_{j\in R_i}v_{ij} v_{il_i}\right] \le  v_{il_i} \E[v_i(R_i + l_{i})] = v_{i l_i} f_i(\by).$$ 
By Chebyshev's inequality, we have $$\Pr\left[f_i(R_i + l_{i})\le \frac{f_{i}(\by)}{2}\right] \le \frac{\Var[f_i(R_i + l_{i})]}{(f_{i}(\by)/2)^2}\le \frac{4v_{i l_i}}{f_{i}(\by)}.$$
Therefore, using the fact that $f_i(\by) \geq v_{i l_i}$ with probability $1$,
$$\E\left[\frac{f_{i}(\by)}{f_i(R_i + l_{i})} \Big| \by \right] \le \frac{f_{i}(\by)}{f_{i}(\by)/2} \cdot \Pr\left[f_i(R_i + l_{i}) > \frac{f_{i}(\by)}{2}\right]  + \frac{f_{i}(\by)}{v_{i, l_i}}\cdot\Pr\left[f_i(R_i + l_{i})\le \frac{f_{i}(\by)}{2}\right]  \le 2+4=6. $$ 
Combining the two rounding steps, and using $v_i(R_i+l_i) \geq f_i(R_i+l_i)$, we have
$$  \E\left[\frac{v^+_i(\bx)}{v_i(R_i + l_{i})} \Big| S_i \right] = 
 \E\left[\frac{v^+_i(\bx)}{f_{i}(\by)} \E\left[\frac{f_{i}(\by)}{v_i(R_i + l_{i})}\bigg|\by\right] \Big| S_i \right] \leq 
 6 \cdot \E\left[ \frac{v^+_i(\bx)}{f_i(\by)} \Big| S_i \right]  \leq 42.$$
 Now we can remove the conditioning on $S_i$, and obtain $\E\left[\frac{v^+_i(\bx)}{v_i(R_i + l_{i})} \Big| S_i \right] \leq 42$, for every $i \in \cA'$. Finally, we sum up over $i \in \cA'$ and use (\ref{eq:local-opt-bound}):
$$ \sum_{i \in \cA'} \E\left[ \frac{v^+_i(\bx^*_i)}{v_i(R_i+l_i)}\right] 
= \sum_{i \in \cA'} \frac{v^+_i(\bx^*_i)}{v^+_i(\bx_i)} \E\left[  \frac{v^+_i(\bx)}{v_i(R_i+l_i)} \right]
\leq 42 \sum_{i \in \cA'} \frac{v^+_i(\bx^*_i)}{v^+_i(\bx_i)} \leq 84 n.  $$

\end{proof}

\subsection{Matching recombination}

In this section we show how to allocate the remaining unassigned items, i.e. items in $\cH$ and those large items $l_i$ which randomized rounding does not handle well. To achieve our goal, we borrow two lemmas from previous work. Lemma 5 tells us that we lose at most a constant factor if we only allocate items in $\cH$ via matching. Lemma 6 is a relatively sophisticated tool, called `matching recombination'. The lemma shows that for any fractional solution $\by$ and any matching $\pi:\cA \rightarrow \cH$ (imagine the optimal matching on top of $\by$), there is another matching $\rho: \cA \rightarrow \cH$ such that the value of $(\by, \rho)$ is comparable to the value of $(\by,\pi)$, and for each agent, either the item matched in $\rho$ has a significant value, or there is no item outside of $\cH$ which has a significant value. We will show that, in either case, we can safely throw away the large items $l_i$ and won't lose too much. 


\

(CAREFUL: The lemma in \cite{LiV22} is not formulated with $v^+_i(\by_i)$; we need to justify this.)

\begin{lemma}[Lemma 6 in \cite{LiV22}]
\label{lem:rematching}
Let $\bx^*$ be the optimal solution of (Mixed-Concave Relaxation), i.e.~$\bx^*_i = \by^*_i + \b1_{H^*_i}$ where $\by^* \in [0,1]^{\cA \times \cG}$ is a feasible solution of (Log-Concave Relaxation) and $(H^*_1,\ldots,H^*_n)$ is a partition of $\cH$.
Let $\by' \in [0,1]^{\cA \times \cG}$ be an arbitrary fractional solution, satisfying
$$ \frac{1}{n} \sum_{i \in \cA'} \frac{v_i^+(\by^*_i)}{v_i^+(\by'_i)} \leq \beta $$
and $\by'_i = 0$ for $i \notin \cA'$.
Then there is a matching $\pi:\cA \rightarrow \cH$ such that 
$$ NSW(\by',\pi) = \left(\prod_{i \in \cA} v^+_i(\by'_i + \b1_{\pi(i)}) \right)^{1/n}
 \geq \frac{1}{\beta+1} \left( \prod_{i \in \cA} v^+_i(\bx^*_i) \right)^{1/n} = \frac{1}{\beta+1} \ OPT.$$
\end{lemma}

\begin{lemma}[Lemma 6.1 in \cite{garg2020approximating}, Lemma 8 in \cite{LiV22}]
\label{lem:matching}
Let $d \geq 2$.
Let $\tau:\cA \rightarrow \cG$ be the matching maximizing $\prod_{a \in \cA} v_i(\tau(a))$, $\cH = \tau(\cA)$ the items allocated in this matching. Let $\by \in [0,1]^{\cA' \times \cG'}$ and let $\pi: \cA \rightarrow \cH$ be any matching. Then there is a matching $\rho: \cA \rightarrow \cH$ such that
$$ \NSW(\by,\rho) \geq \frac{1}{d+2} \NSW(\by, \pi) $$
and for every agent $a \in \cA$,
\begin{enumerate}
    \item [(i)] either $v_a(\rho(a)) \geq \frac{1}{d} v_a^+(\by_a)$ 
    (in which case the $\rho$-matching item itself recovers a constant fraction of agent $a$'s value)
    
    \item [(ii)] or for every item $j \in \cG'$, $v_a(j) < \frac{1}{d} v_a^+(\by_a)$  
    (in which case there are no items with large contributions to $v_a^+(\by_a)$).
\end{enumerate}




\begin{proof}[Proof of Theorem 1]
Given the solution $(R+l) = (R_1+l_1,\ldots,R_n+l_n)$ and the matching $\pi$ provided by Lemma~\ref{lem:rematching}, satisfying
$$ \NSW(R+l,\pi) \geq \frac{1}{90} OPT, $$
let $\rho$ be the matching provided by Lemma~\ref{lem:matching} with parameter $d = 2$. This matching satisfies
$$ \NSW(R+l,\rho) \geq \frac{1}{4} \NSW(R+l, \pi) \geq \frac{1}{360} OPT $$
and for every agent $i \in \cA$, either (i) $v_i(\rho(i)) \geq \frac{1}{2} v_i^+(R_i+l_i)$  or (ii) for every item $j \in \cG' = \cG\backslash\cH$, $v_i(j) < \frac{1}{2} v_i(R_i +l _i)$. 

For every agent $i\in\cA$, if (i) is the case, then we know that 
$$v_i(R_i + \rho(i))\ge v_i(\rho(i)) \ge \frac{1}{4}\left(v_i(R_i)+v_i(l_i)+v_i(\rho(i))\right)\ge\frac{v_i(R_i+l_i+\rho(i))}{4}.$$ 
Otherwise in case (ii), we have 
\begin{align*}
    v_i(R_i + \rho(i))&\ge v_i(R_i+l_i+\rho(i)) - v_i(l_i) \\
    &\ge v_i(R_i +l _i + \rho(i)) - \frac{v_i(R_i +l _i)}{2}  \\ &\ge\frac{v_i(R_i +l _i + \rho(i))}{2}.
\end{align*}

In conclusion, we know that for any agent $i\in\cA$, 
$$v_i(R_i + \rho(i)) \ge \frac{v_i(R_i+l_i+\rho(i))}{4}.$$ 
Therefore, we obtain
$$ \left( \prod_{i \in \cA} v_i(R_i + \rho(i)) \right)^{1/n} \ge 
\frac{1}{4}  \NSW(R+l, \rho) \geq \frac{OPT}{1440}.$$

\end{proof}
\end{lemma}


